TrollSpot: Detecting misbehavior in commenting platforms

Commenting platforms, such as Disqus, have emerged as a major online communication platform with millions of users and posts. Their popularity has also attracted parasitic and malicious behav- iors, such as trolling and spamming. There has been relatively little research on modeling and safeguarding these platforms. As our key contribution, we develop a systematic approach to detect malicious users on commenting platforms focusing on having: (a) interpretable, and (b) fine-grained classification of malice. Our work has two key novelties: (a) we propose two classifications methods, with one following a two stage approach, which first maps observ- able features to behaviors and then maps these behaviors to user roles, and (b) we use a comprehensive set of 73 features that span four dimensions of information. We use 7 million comments during a 9 month period, and we show that our classification methods can distinguish between benign, and malicious roles (spammers, trollers, and fanatics) with a 0.904 AUC. Our work is a solid step to- wards ensuring that commenting platforms are a safe and pleasant medium for the exchange of ideas.

==> 401_features-NOTUSED.tex <==
\subsection{Features}

\textbf{Engagement features}. We take the total number of engagements of a user and the statistical result (AVG, MIN and MAX) of their duration and intensity. It has been shown that high intensity engagements usually imply a potential misbehavior as we discuss before. 
Maintaining a short and regular duration on all engagements also suggest a possibility of a spammer.

\textbf{Social features}. The degree of user, number of triangles and number of maximal cliques in Collaboration Graph are taking into account. We use these features to capture users local connectivity to understand how breadth and depth they interact with others. Considering trolls may spend more times putting provocative comments on multiple articles which results in having higher degree than benign users.

\textbf{Temporal features}. We simply take the standardizing number of comments users made in each hour of the day as features. 

\textbf{Linguistic features}. Number of words, sentences, percentage of capital letters, text readability and number of URLs in comment are used to characterized the quality of comments, and the statistic result are then used as features to identify misbehaving users.
The badness of a user could easily be spotted from the content of the comment they made. It has been shown that misbehavior users would make less readability comments \reminder{reference}, number of words and URLs would also be the sign of spammers.

